Towards Open Ad Hoc Teamwork Using Graph-based Policy Learning

Ad hoc teamwork is the challenging problem of designing an autonomous agent which can adapt quickly to collaborate with teammates without prior coordination mechanisms, including joint training. Prior work in this area has focused on closed teams in which the number of agents is fixed. In this work, we consider open teams by allowing agents with different fixed policies to enter and leave the environment without prior notification. Our solution builds on graph neural networks to learn agent models and joint-action value models under varying team compositions. We contribute a novel action-value computation that integrates the agent model and joint-action value model to produce action-value estimates. We empirically demonstrate that our approach successfully models the effects other agents have on the learner, leading to policies that robustly adapt to dynamic team compositions and significantly outperform several alternative methods.

==> archived/intro2-old.tex <==
\begin{document}
\section{Introduction}
Many real world problems require agents to perform tasks in the presence of other agents. Consider an autonomous car driving through an urban street populated with pedestrians and other vehicles. Multi-agent reinforcement learning (MARL) tackles these problems by jointly training a set of agents with shared learning procedures assuming knowledge over each agent’s reward function ~\citep{lowe2017multi, foerster2018a, DBLP:conf/icml/RashidSWFFW18}. Knowledge over other agents rewards is in many setting an unrealistic assumption. Take the urban street example, other vehicles can be driven by humans or be produced by other manufacturers, making joint training with MARL impossible. When executing tasks in which agent types are encountered that are not seen during joint training, MARL approaches are unlikely to generalize their training performance.

By contrast, opponent modelling techniques ~\citep{he2016opponent,DBLP:conf/icml/RaileanuDSF18,DBLP:conf/iclr/TacchettiSMZKRG19,grover2018learning,rabinowitzToM} use the observed behavior of an uncontrolled agent to learn a representation of it. This representation is often interpreted as a goal or intention of the agent ~\citep{DBLP:conf/icml/RaileanuDSF18,rabinowitzToM}. Most of the literature has been focused on different methodologies to learn agent representations ~\citep{DBLP:conf/icml/RaileanuDSF18,grover2018learning,rabinowitzToM}, but made unsatisfactory progress considering the question of how to integrate a learned representation to improve the decision making of the controlled agent ~\citep{DBLP:conf/iclr/TacchettiSMZKRG19}. We argue that for the controlled agent the decisive step is to understand how other agents expected actions will influence his reward. Any architecture that has this premise incorporated as an inductive bias, should outperform a simple concatenation approach that adds an agent representation as additional input into a neural net.  

Leveraging factored joint-action value models, one can disentangle the effect an agents action or the joint action of a group of agents have on the return. Since we are not able to control the actions other agents choose, the uncertainty in their actions needs to be accounted for. Estimating the policy of other agents via an agent model lets us marginalize out their effect on the action value of the controlled agent, leading to a better action value estimate. This provides a novel methodology to compute action values which can be leveraged within any reinforcement learning algorithm that makes use of such.

We show empirically that MARL approaches fail to generalize to settings in which an agent has to interact with unseen agents. In this setting GPL is able to outperform prior opponent modelling techniques that are based on DQN or actor-critic methods. Interestingly, we observe that our methods allows agents to "pick up skills" from other agents, enabling more sample efficient learning. We are the first opponent modelling paper that tests their approach in open environments, where agents with diffrerent policies can enter and leave during an episode at training as well as test time.


\end{document} 

==> archived/intro2.tex <==
\begin{document}
\section{Introduction}
Many real world problems require agents to perform tasks in the presence of other agents. Consider an autonomous car driving through an urban street populated with pedestrians and other vehicles. Multi-agent reinforcement learning (MARL) tackles these problems by jointly training a set of agents with shared learning procedures assuming knowledge over each agent’s reward function ~\citep{lowe2017multi, foerster2018a, DBLP:conf/icml/RashidSWFFW18}. Knowledge over other agents rewards is in many setting an unrealistic assumption. Take the urban street example, other vehicles can be driven by humans or be produced by other manufacturers, making joint training with MARL impossible. When executing tasks in which agent types are encountered that are not seen during joint training, MARL approaches are unlikely to generalize their training performance.

By contrast, opponent modelling techniques ~\citep{he2016opponent,DBLP:conf/icml/RaileanuDSF18,DBLP:conf/iclr/TacchettiSMZKRG19,grover2018learning,rabinowitzToM} use the observed behavior of an uncontrolled agent to learn a representation of it. Most of the literature has been focused on different methodologies to learn agent representations ~\citep{DBLP:conf/icml/RaileanuDSF18,grover2018learning,rabinowitzToM}, which are then used to augment the input of a policy network or value network. These methods have lead to more stable ~\citep{he2016opponent} and more sample efficient ~\citep{DBLP:conf/iclr/TacchettiSMZKRG19,grover2018learning} training, but did not outperform baseline in terms of final reward. We argue that for the controlled agent the decisive step is to understand how other agents expected actions will influence his reward. Any architecture that has this premise incorporated as an inductive bias, should outperform a simple concatenation approach that adds an agent representation as additional input into a neural net.

We study the use of opponent models to train a single agent to interact in a multi-agent environments. Other agents that are present in the environment are non-learning, but can follow a variety of different policies. Each non-controlled agent can leave and enter the environment \textit{at any timestep during an episode} and can be either opposing to the learning agent or cooperative. For the learning agent to achieve high reward in such an environment it is of importance not to misattribute the cause of a reward signal to one of his actions while the actions of other were responsible for it. In a game in which  it is beneficial to shoot other agents, misattributing reward from successful shots of teammates to its own random action may inable the agent to discover that shooting opponents is a useful action. Misattribution can lead to slower learning, i.e. needing more experience learning the true mechanism by which to obtain reward or can cause the agent not to learn at all, i.e. never understanding the mechanism by which reward can be obtained. 


While joint action value models have been widely adapted in MARL research ~\citep{DBLP:conf/icml/RashidSWFFW18,DBLP:conf/atal/SunehagLGCZJLSL18}, there usage for single-agent learner problems has not been explored yet. In graph-based policy learning (GPL) we leverage factored joint-action value models to disentangle the effect an agents action or the joint action of a group of agents have on the return of the learning agent. Since we are not able to control the actions other agents choose, the uncertainty in their actions needs to be accounted for. Estimating the policy of other agents via an agent model lets us marginalize out their effect on the action value of the controlled agent, leading to a better action value estimate. This provides a novel methodology to compute action values which can be leveraged within any reinforcement learning algorithm that makes use of such.

We show empirically that MARL approaches fail to generalize to settings in which an agent has to interact with unseen agents. In this setting GPL is able to outperform prior opponent modelling techniques in terms of final reward achieved during training and reward achieved when generalizing to test environments with a number of agents unseen during training. Interestingly, we observe that our methods allows agents to \textit{pick up skills} from other agents, enabling more sample efficient learning. Out contributions are summarized below:


\begin{itemize}[leftmargin=*]
    \item We provide a novel methodology to compute action values in the presence of other agents, that lets agents disentangle the effects other agents actions and its own actions have on reward.
    \item We show that our method outperforms prior opponent modelling techniques in terms of final reward and generalisation to unseen number of agents at test time on three environments. 
    \item We are the first opponent modelling paper that tests their approach in open environments, where agents with different policies can enter and leave during an episode at training as well as test time. 
\end{itemize}




\end{document} 

==> archived/method_description.tex <==
\begin{document}
\section{Graph-based Policy Learning}
In this section, we introduce the general features of GPL and the motivation behind their usage for estimating an OSBG's optimal policy. We also describe the neural network architectures and the learning procedures used for implementing each feature. A general overview of GPL's architecture is provided in Figure~\ref{} while the complete learning pseudocode is given in Appendix~\ref{}.

\subsection{General Features of GPL}
\label{GeneralFeatures}
In an OSBG, agents' joint actions inherently affect the learner's returns through the reward and next states experienced by the learner. Disregarding other agents' actions while learning, as in the case of single-agent RL, may have adverse effects towards the learned policy's performance. Imagine a soccer domain where a learner is rewarded whenever its team scores a goal. There are instances when the learner's action has no impact towards teammates scoring goals, such as when the learner is far from the scorer's position. In this case, a learner using simple Q-learning ~\citep{watkins1992q} will increase the action-values of its previous action after observing the rewards, even if the action itself was irrelevant for generating the reward.

We prevent the aforementioned learning problem by including \textit{joint action value} estimation as a feature of GPL. The joint action value of a policy, $Q_{\pi}(s, a)$, is defined as :
\begin{equation}\mathbb{E}_{a^{i}_{t} \sim \pi, a^{-i}_{t}\sim\boldsymbol{\pi}^{-i}, P}\AverX[\bigg]{\sum_{t=0}^{\infty} \gamma^{t}r(s_{t}, a_{t})\given s_{0}=s, a_{0}=a}.
\label{JointActionReturns}
\end{equation}
In contrast to Equation~\ref{ActionReturns}, this joint action value denotes the learner's expected returns after the joint agent-action $a$ at $s$. Estimating the joint action value forces GPL to take into account others' actions into its returns. This prevents the learner from only crediting its own action if it has minimal contribution towards the observed rewards.

Unlike action-values, joint action values introduces a problem for action selection. Being optimistic by choosing $a^{i}$ from the joint agent-action with maximum value yields suboptimal policies. Other agents may choose actions that does not maximize the learner's returns. However, we show using Equation~\ref{Marginalisation} that the joint action value estimates can be used to compute $\bar{Q}^{\pi}(s_{t},a_{t}^{i})$, which facilitates greedy action selection for computing the optimal policy. Since $\pi^{-i}_{t}(a^{-i}_{t}|s_{t}, a^{i}_{t})$ in Equation~\ref{Marginalisation} is unknown to the learner, it is estimated by GPL's \textit{agent modelling} feature. We provide the proof of Equation~\ref{Marginalisation} in Appendix~\ref{}.
\begin{equation}
    \bar{Q}_{\pi}(s_{t},a_{t}^{i}) = \mathbb{E}_{a_{t}^{-i}\sim\boldsymbol{\pi}_{t}^{-i}(.|s_{t},a_{t}^{i})}\AverX{Q_{\pi}(s_{t},a)|a^{i}=a_{t}^{i}}
    \label{Marginalisation}
\end{equation}

Another feature of GPL is the \textit{type inference} feature. In an OSBG, types affects $Q(s,a)$ and $\pi^{-i}(a^{-i}|s, a^{i})$ by determining other agent's immediate actions and long term behaviour. Estimation of $Q(s,a)$ and $\pi^{-i}(a^{-i}|s, a^{i})$ must subsequently take agent types as input. However, agent types are unknown and must be inferred from agents' observed behaviour by this feature.

%

The aforementioned GPL features are finally implemented using neural networks that may facilitate efficient computation of $\bar{Q}^{\pi^{*}}(s,a^{i})$ while handling environment openness. GPL enables efficient computation of $\bar{Q}^{\pi^{*}}(s,a^{i})$ by imposing a simple factorization of the joint action value. On the other, environment openness is handled by implementing several features with GNNs.

\subsection{The GPL Architecture}

\textbf{Type inference:} In the absence of knowledge over the inherent type space of an OSBG, GPL's assumes that types can be represented as fixed-length vectors. Since it may require reasoning over agent's behaviour over an extended period of time, type inference is implemented as LSTMs~\citep{hochreiter1997long}.
The LSTM takes the observed state ($u_{t}$) and agent-specific information ($x^{i}_{t}$) at time $t$ to produce a hidden-state vector as an agent's type embedding. Full details on the computation of type vectors can be found in Appendix~\ref{GPLpreprocessing}. GPL uses the type embeddings as input for the joint action value and agent modelling network. Although the joint action value and agent modelling feature may use the same type inference network, separate networks are used to prevent both model's gradients from interfering against each other during training.

\textbf{Joint action value estimation:} The learner's joint action value is represented as a fully connected Coordination Graph~\citep{guestrin2002coordinated} (CGs). A fully connected CG factorizes the joint action value as:\begin{equation}\label{JointActionValueComputation}\
    Q_{\beta,\delta}(s_{t}, a_{t}) = \sum_{j\in{N_{t}}} Q^{j}_{\beta}(a^{j}_{t}|s_{t}) + \sum_{\substack{j,k\in{N_{t}}\\j\neq{k}}}Q^{j,k}_{\delta}(a_{t}^{j},a_{t}^{k}|s_{t}),
\end{equation}with $Q^{j}(a^{j}|s)$ and $Q^{j,k}(a^{j},a^{k}|s)$ being the singular and pairwise utility terms respectively. The singular and pairwise utility terms are computed using MLPs parameterized by $\beta$ and $\delta$ respectively. When computing a utility term, both MLPs receives type embeddings of the learner and agents associated to the term as input, which enables each term to the associated agent's contribution towards the learner's returns. Details on the computation of the utility terms are provided in Appendix~\ref{}.

We represent our joint action value as CGs for three reasons. First, CGs impose a joint action value factorization that facilitates an efficient action-value computation. We further elaborate the computational complexity of computing action-values with CGs when discussing about GPL's action-value computation. Second, CGs are implementable as GNNs~\citep{DCG}, which makes it a good fit for handling openness. Third, CG's value factorization enables GPL to model the contribution of other agents' actions towards the returns. Specifically, $Q^{j}(a^{j}|s)$ estimates the contribution of agent $j$ while $Q^{j,k}(a^{j},a^{k}|s)$ estimates the contribution of agent $j$ and $k$ as a pair.

\textbf{Agent modelling:} GPL uses the Relational Forward Model (RFM) architecture~\citep{DBLP:battaglia} for agent modelling. As a GNN, RFM has been demonstrated to be a good fit for agent modelling in open teams. Assuming $\zeta$ denotes its parameters, the RFM network receives agent type embeddings, $\theta_{q}$, as its node input to compute a fixed-length embedding, $\bar{n}$, for each agent. Assuming $a^{j}$ is the action taken by $j$ in the joint agent-action $a^{-i}$, we use each agent's updated embedding to approximate $\pi^{-i}(a^{-i}|s,a^{i})$ as :
\begin{equation}\label{GNNequations}
q_{\eta,\zeta}(a^{-i}|s, a^{i}) = \prod_{j\in{-i}}\textrm{Softmax}(MLP_{\eta}(\bar{n}_{j}))(a^{j}),
\end{equation}with $\eta$ being the parameter of an MLP that transforms the updated agent embeddings. 

\textbf{Action value computation:} Evaluating Equation~\ref{Marginalisation} can be inefficient in larger teams. This is because the number of evaluated joint action value terms increases exponentially relative to the team size. For example, a team of 10 agents which may choose from 5 possible actions requires the evaluation of $5^{10}$ joint action terms. By contrast, a more efficient action-value computation arises from factorizing the joint action value network and using RFM-based agent modelling networks. B substituting Equation~\ref{JointActionValueComputation} and~\ref{GNNequations} to compute Equation~\ref{Marginalisation}, we obtain the following Equation as our action-value estimate :
\begin{align}\label{SingleActionValue}
\begin{split}
\bar{Q}(s_{t}, a^{i}) & = Q^{i}_{\beta}(a^{i}|s_{t})  \\
& + \sum_{ \mathclap{\substack{a^{j}\in{A_{j}},  j\neq{i}}}}\big(Q^{j}_{\beta}(a^{j}|s_{t})+Q^{i,j}_{\delta}(a^{i}, a^{j}|s_{t})\big)q_{\zeta,\eta}(a^{j}|s_{t}) \\
&+ \sum_{\mathclap{\substack{a^{j}\in{A_{j}},a^{k}\in{A_{k}}, j, k\neq{i}}}}Q^{j,k}_{\delta}(a^{j}, a^{k}|s_{t})q_{\zeta,\eta}(a^{j}|s_{t})q_{\zeta,\eta}(a^{k}|s_{t}).
\end{split}
\end{align}Unlike Equation~\ref{Marginalisation}, Equation~\ref{SingleActionValue} is defined in terms of singular and pairwise action terms. In this case, the number of terms that needs to be computed only increases quadratically as the team size increases. Furthermore, the computation of the required terms can be efficiently done in parallel with existing GNN libraries.


\textbf{Model optimization:} Given a dataset of other agents' actions at different states, we train the agent modelling network to estimate $\pi(a^{-i}|s,a^{i})$ through supervised learning by minimizing the negative log likelihood of its parameters,
\begin{align}\label{ActionModelLoss}
\begin{split}
    L_{\zeta, \eta} &= -\text{log}(q_{\zeta,\eta}(a^{-i}|s,a^{i})).
\end{split}
\end{align}On the other hand, GPL's joint-action value network is trained using a slight modification of asynchronous Q-Learning~\citep{mnih2016asynchronous}. Unlike off-the-shelf Q-Learning, we use the joint action value as the predicted value instead of the action-values. The loss function for the joint action value network is then defined as,
\begin{equation}
    L_{\beta,\delta} = \dfrac{1}{2}\left(Q_{\beta,\delta}\left(s_{t}, a_{t}\right)-r_{t}-\gamma \text{max}_{a^{i}}\bar{Q}\left(s_{t+1},a^{i}\right)\right)^2,
    \label{ValueLoss}
\end{equation}
which is similar to the loss function used by Q-Learning.

\end{document}

==> archived/problem_formulation.tex <==
\begin{document}
\section{Problem formulation}

In this section, we formalize the problem of open ad hoc teamwork by extending the Stochastic Bayesian Game model~\citep{albrecht2016belief} to allow for openness. We subsequently define the optimal policy, which must be estimated by any learning approach for open ad hoc teamwork.

\subsection{Open Stochastic Bayesian Games (OSBG)}
Open ad hoc teamwork requires an agent to interact with other agents that have unknown policies, and may enter or leave the environment based on the environment state and actions of agents.

In our definition of OSBGs, we represent agents and their action of choice as a set of agent-action pairs. Formally, let $N$ be a set of agents and $A$ be the individual action space, which is assumed to be the same for all agents. The joint agent-action space, which represents the set of valid agent-action combinations, is defined as $\boldsymbol{NA}=\{a|a\in\mathcal{P}(N \times A), \forall{(i,a^{i}),(j,a^{j})} \in a: i=j \Rightarrow a^{i}=a^{j}\}$, where $\mathcal{P}$ denotes the power set. The elements of $\boldsymbol{NA}$ is referred to as \emph{joint agent-actions} and is used to represent the action selected by agent $i$ in $a$. Note that the condition in the definition of $\boldsymbol{NA}$ imposes agents in $a \in \boldsymbol{NA}$ to only choose a single action for valid action selections. 

The OSBG definition also use \textit{types} to represent the behavioural model of an agent, which is assumed to be unknown to others. With $\Theta$ and $S$ denoting the set of possible types and states respectively, each agent chooses their actions via the policy function, $\pi:S \times \mathcal{P}(N) \times \Theta \mapsto \Delta(A)$, based on the current state, set of existing agents, and the agent's own type. We subsequently denote the set of valid agent-type assignments as $\boldsymbol{N\Theta}=\{\theta|\theta\in\mathcal{P}(N \times \Theta), \forall{(i,\theta^{i}),(j,\theta^{j})}\in\theta: i=j\Rightarrow\theta^{i}=\theta^{j}\}$. We refer to $\theta \in \boldsymbol{N\Theta}$ as the \emph{joint agent-types} and use $\theta^{i}$ to denote the type of agent $i$ in $\theta$. 

We model the decision making problem in open ad hoc teamwork as an \emph{Open Stochastic Bayesian Game} (OSBG), which is a 6-tuple $(N,S,A,\Theta,R,P)$ with $N,S,A$, and $\Theta$ already defined above. In an OSBG, we assume control over a single agent that is always present in the environment. The reward function, $R:S\times \boldsymbol{NA} \times \Theta \mapsto \mathbb{R}$, is a scalar used as a learning signal by the learner. Note that the reward function is dependent of other agents' actions. The transition function $P: S \times \boldsymbol{NA} \mapsto \Delta(S \times \boldsymbol{N\Theta})$ determines the probability of the next state and the next joint agent-types, given the current state and joint agent-actions. Although the transition function allows agents to have changing types, our current work assumes that the type of an agent stays fixed between entering and leaving the environment. 

Under an OSBG, the game starts by sampling an initial state, $s_{0}$, and an initial set of agents, $N_{0}$, with associated types, $\theta_0^i$ with $i\in N_0$, from a starting distribution $P_{0} \in \Delta(S \times \boldsymbol{N\Theta})$. At state $s_{t}$, agents $N_{t} \subseteq N$ with types $\theta_t^i,i \in N_t$ exist in the environment and choose their actions $a^{i}_{t}$ by sampling from $\pi$. As a consequence of the selected joint agent-actions, the learner receives a reward computed through $R$. Finally, the next state $s_{t+1}$ and the next set of existing agents $N_{t+1}$ and types are sampled from $P$ given $s_t$ and joint agent-actions.

\subsection{Optimal Policies for OSBGs}
To solve an OSBG, a learning approach must estimate the optimal policy for the learning agent, $i$, as defined below: 

\begin{cdef}
Let the joint actions of agents other than $i$ at time $t$ be denoted by $a^{-i}_{t}$ and the joint policy of agents other than $i$ at time $t$ by $\boldsymbol{\pi}^{-i}_{t}$. Given a discount factor $\gamma$, we define the action-value of policy $\pi$ , $\bar{Q}_{\pi}(s,a^{i})$, as :
\begin{equation}\mathbb{E}_{a^{i}_{t} \sim \pi, a^{-i}_{t}\sim\boldsymbol{\pi}^{-i}_{t}, P}\AverX[\bigg]{\sum_{t=0}^{\infty} \gamma^{t}r(s_{t}, a_{t})\given s_{0}=s, a^{i}_{0}=a^{i}},
\label{ActionReturns}
\end{equation}
which denotes the expected discounted returns after the learner executes $a^{i}$ at $s$. A policy, $\pi^{*}$, is then optimal if :
\begin{equation}
    \forall{\pi, s, a^{i}}, \bar{Q}_{\pi^{*}}(s,a^{i}) \geq \bar{Q}_{\pi}(s,a^{i}).
\end{equation}
Given $\bar{Q}_{\pi^{*}}(s,a)$, an OSBG is solved by always choosing $a^{i}$ with the highest action-value at $s$. 
\end{cdef}

% \begin{cdef}
% Let the joint actions of agents other than $i$ at time $t$ be denoted by $a^{-i}_{t}$ and the joint policy of agents other than $i$ at time $t$ by $\boldsymbol{\pi}^{-i}_{t}$.
% Given a discount factor $\gamma$, the joint action value function for agent $i$'s policy $\pi$, $Q_{\pi,i}(s,a)$,
% %which computes $i$'s expected discounted return in an OSBG after the execution of joint agent-action $a$ in state $s$ and thereafter following $\pi$
% is defined as:
% \begin{equation}\mathbb{E}_{a^{i}_{t} \sim \pi, a^{-i}_{t}\sim\boldsymbol{\pi}^{-i}_{t}, P}\AverX[\bigg]{\sum_{t=0}^{\infty} \gamma^{t}u^{i}(s_{t}, a_{t})\given s_{0}=s, a_{0}=a}
% \label{JointReturns}
% \end{equation}
% \end{cdef}

% Note that $Q_{\pi,i}$ is defined over $\boldsymbol{NA}$ in contrast to the usual definition over the joint action space and the policies of other agents depend on time $t$ since different agents can be present at different timesteps. For an agent $i$, solving an OSBG is equivalent to finding an optimal policy, $\pi^{*}$, where $\forall{\pi},s,a: Q_{\pi^{*},i}(s,a)\geq{Q_{\pi,i}}(s,a)$. Under the optimal policy agent $i$ chooses actions that maximize the action value, $\bar{Q}^{*}$:
% \begin{align} \label{Marginalisation}
% \begin{split}
% \pi^{*}(s) &= \text{argmax}_{a^{i}}  \bar{Q}^{*}_{i}(s,a^{i}), \\ \bar{Q}^{*}(s,a^{i})  &=\mathbb{E}_{a^{-i}\sim\boldsymbol{\pi}^{-i}}\AverX{Q_{\pi^{*},i}(s,\{(i,a^{i}),(-i,a^{-i})\})}. 
% \end{split}
% \end{align}

\end{document}

==> archived/problem_formulation2.tex <==
\begin{document}
\section{Problem formulation}

In this section, we formalize the problem of controlling a single agent acting in an environment with other agents present. Other agents have different types and can leave and enter the environment at any timestep. Our formulation builds upon and extends the Stochastic Bayesian Game model~\citep{albrecht2016belief} to allow for openness. 

\subsection{Open Stochastic Bayesian Games (OSBG)}
One goal of the problem formulation is not to assume a fixed number of agents that can enter and leave the environment. Openness in real world situations often means that the maximum number of agents is not previously known. Not restricting the number of agents to a fixed number prevents us from defining joint action and type spaces via tuples. Therefore we define a novel joint agent-action and joint agent-type space. Formally, let $N$ be a possibly infinite set of agents and $A$ be their shared action space. The joint agent-action space, which represents the set of valid agent-action combinations, is defined as $\boldsymbol{NA}=\{a|a\in\mathcal{P}(N \times A), \forall{(i,a^{i}),(j,a^{j})} \in a: i=j \Rightarrow a^{i}=a^{j}\}$, where $\mathcal{P}$ denotes the power set, elements $a\in \boldsymbol{NA}$ are called \emph{joint agent-actions} and $a^{i}$ refers to the action selected by agent $i$ in $a$. The condition in the definition of $\boldsymbol{NA}$ imposes agents in $a \in \boldsymbol{NA}$ to only choose a single action

The OSBG definition uses \textit{types} to represent the behavioural model of an agent, which is assumed to be unknown to others. With $S$ denoting the state space, each agent chooses their actions via the policy function, $\pi:S \times \mathcal{P}(N) \times \Theta \mapsto \Delta(A)$, based on the current state, set of existing agents, and its own type. Given type space, $\Theta$, we denote the set of valid agent-type assignments as $\boldsymbol{N\Theta}=\{\theta|\theta\in\mathcal{P}(N \times \Theta), \forall{(i,\theta^{i}),(j,\theta^{j})}\in\theta: i=j\Rightarrow\theta^{i}=\theta^{j}\}$. We refer to $\theta \in \boldsymbol{N\Theta}$ as the \emph{joint agent-types} and use $\theta^{i}$ to denote the type of agent $i$ in $\theta$. 

We model the decision making problem in open ad hoc teamwork as an \emph{Open Stochastic Bayesian Game} (OSBG), which is a 6-tuple $(N,S,A,\Theta,R,P)$ with $N,S,A$, and $\Theta$ already defined above. In an OSBG, we assume control over a single agent that is always present in the environment. The reward function, $R:S\times \boldsymbol{NA} \times \Theta \mapsto \mathbb{R}$, is a scalar used as a learning signal by the learner. We parameterize the reward function with other agents' actions to model the way it affects the learner's ability to perform tasks. The transition function $P: S \times \boldsymbol{NA} \mapsto \Delta(S \times \boldsymbol{N\Theta})$ determines the probability of the next state and the next joint agent-types, given the current state and joint agent-actions. Although OSBGs allows agents to have changing types, our current work assumes that the type of an agent stays fixed between entering and leaving the environment. 

Under an OSBG, the game starts by sampling an initial state, $s_{0}$, and an initial set of agents, $N_{0}$, with associated types, $\theta_0^i$ with $i\in N_0$, from a starting distribution $P_{0} \in \Delta(S \times \boldsymbol{N\Theta})$. At state $s_{t}$, agents $N_{t} \subseteq N$ with types $\theta_t^i,i \in N_t$ exist in the environment and choose their actions $a^{i}_{t}$ by sampling from $\pi$. As a consequence of the selected joint agent-actions, the learner receives a reward computed through $R$. Finally, the next state $s_{t+1}$ and the next set of existing agents $N_{t+1}$ and types are sampled from $P$ given $s_t$ and joint agent-actions.

\subsection{Optimal Policy for OSBGs}
To solve an OSBG, a learning approach must estimate the optimal policy for the learning agent, $i$, as defined below: 

\begin{cdef}
Let the joint actions of agents other than $i$ at time $t$ be denoted by $a^{-i}_{t}$ and the joint policy of agents other than $i$ at time $t$ by $\boldsymbol{\pi}^{-i}_{t}$. Given a discount factor $\gamma$, we define the action-value of policy $\pi$ , $\bar{Q}_{\pi}(s,a^{i})$, as :
\begin{equation}\mathbb{E}_{a^{i}_{t} \sim \pi, a^{-i}_{t}\sim\boldsymbol{\pi}^{-i}_{t}, P}\AverX[\bigg]{\sum_{t=0}^{\infty} \gamma^{t}r(s_{t}, a_{t})\given s_{0}=s, a^{i}_{0}=a^{i}},
\label{ActionReturns}
\end{equation}
which denotes the expected discounted returns after the learner executes $a^{i}$ at $s$. A policy, $\pi^{*}$, is then optimal if :
\begin{equation}
    \forall{\pi, s, a^{i}}, \bar{Q}_{\pi^{*}}(s,a^{i}) \geq \bar{Q}_{\pi}(s,a^{i}).
\end{equation}
Given $\bar{Q}_{\pi^{*}}(s,a)$, an OSBG is solved by always choosing $a^{i}$ with the highest action-value at $s$. 
\end{cdef}

% \begin{cdef}
% Let the joint actions of agents other than $i$ at time $t$ be denoted by $a^{-i}_{t}$ and the joint policy of agents other than $i$ at time $t$ by $\boldsymbol{\pi}^{-i}_{t}$.
% Given a discount factor $\gamma$, the joint action value function for agent $i$'s policy $\pi$, $Q_{\pi,i}(s,a)$,
% %which computes $i$'s expected discounted return in an OSBG after the execution of joint agent-action $a$ in state $s$ and thereafter following $\pi$
% is defined as:
% \begin{equation}\mathbb{E}_{a^{i}_{t} \sim \pi, a^{-i}_{t}\sim\boldsymbol{\pi}^{-i}_{t}, P}\AverX[\bigg]{\sum_{t=0}^{\infty} \gamma^{t}u^{i}(s_{t}, a_{t})\given s_{0}=s, a_{0}=a}
% \label{JointReturns}
% \end{equation}
% \end{cdef}

% Note that $Q_{\pi,i}$ is defined over $\boldsymbol{NA}$ in contrast to the usual definition over the joint action space and the policies of other agents depend on time $t$ since different agents can be present at different timesteps. For an agent $i$, solving an OSBG is equivalent to finding an optimal policy, $\pi^{*}$, where $\forall{\pi},s,a: Q_{\pi^{*},i}(s,a)\geq{Q_{\pi,i}}(s,a)$. Under the optimal policy agent $i$ chooses actions that maximize the action value, $\bar{Q}^{*}$:
% \begin{align} \label{Marginalisation}
% \begin{split}
% \pi^{*}(s) &= \text{argmax}_{a^{i}}  \bar{Q}^{*}_{i}(s,a^{i}), \\ \bar{Q}^{*}(s,a^{i})  &=\mathbb{E}_{a^{-i}\sim\boldsymbol{\pi}^{-i}}\AverX{Q_{\pi^{*},i}(s,\{(i,a^{i}),(-i,a^{-i})\})}. 
% \end{split}
% \end{align}

\end{document}
